Learning to Localize Using a LiDAR Intensity Map

In this paper we propose a real-time, calibration-agnostic and effective localization system for self-driving cars. Our method learns to embed the online LiDAR sweeps and intensity map into a joint deep embedding space. Localization is then conducted through an efficient convolutional matching between the embeddings. Our full system can operate in real-time at 15Hz while achieving centimeter level accuracy across different LiDAR sensors and environments. Our experiments illustrate the performance of the proposed approach over a large-scale dataset consisting of over 4000km of driving.

==> experiments_r.tex <==

\begin{figure*}[tb]
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
\includegraphics[width=0.33\linewidth, trim={1cm 0 0.5cm 0}]{figure/sfo_truck_new_test_linknet_16_5/gil_mean.png}
& \includegraphics[width=0.33\linewidth, trim={1cm 0 0.5cm 0}]{figure/sfo_truck_new_test_linknet_16_5/lateral_hist.png}
& \includegraphics[width=0.33\linewidth, trim={1cm 0 0.5cm 0}]{figure/sfo_truck_new_test_linknet_16_5/lon_hist.png} \\
Error vs Traveling Dist & Lateral Histogram & Longitudinal Histogram
\\\end{tabular}
\caption{Quantatitive Analysis. From left to right: localization error vs traveling distance; lateral error histogram per each timestamp, longitudinal histogram per each step. }
\label{fig:qual-comparison}
\end{figure*}



\section{Experimental Results}
\label{sec:result}






\paragraph{Dataset}
We collected a new dataset comprising  over 5000km of
driving through a variety of urban and highway environments in 
multiple cities/states in North America, collected with two types of \lidar{}
sensors. According to the scenarios we split our datatset into
\textit{Highway-LidarA} and \textit{Misc-LidarB}, where \textit{Highway-LidarA}
contains over 400 sequences for a total of  4,000km  of driving for training and
validation, as well as 359 sequences with 700km of driving  for
testing. All these sequences are collected by a \lidar{} type A.
\textit{Misc-LidarB} contains 79 sequences with 200km of driving 
over a mix of highway and city  collected by
a different \lidar{} type B in a different state. \lidar{}s A and B differ
substantially in their intensity output profiles, as shown in
~\fref{fig:sensor-transfer} (top row).


\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
\includegraphics[width=0.33\linewidth, trim={0 0 0 0}]{figure/icp/lateral_cum.pdf}
& \includegraphics[width=0.33\linewidth, trim={0 0 0 0}]{figure/icp/lon_cum.pdf}
& \includegraphics[width=0.33\linewidth, trim={0 0 0 0}]{figure/icp/trans_cum.pdf} \\

Lateral & Longitudinal & Total Translational
\\\end{tabular}
\caption{Quantatitive Analysis. From left to right: cumulative lateral error; cumulative longitudinal error; cumulative total translational error. }
\label{fig:qual-cum}
\end{figure*}


\paragraph{Experimental Setup}


We randomly collected around 1 million training samples from the training sequences. Each training sample consists of both the BEV intensity image $\cI$
and the 2D \lidar{} intensity map $\cM$. 
\slwang{We aggregate the five most recent online \lidar{} sweeps to generate the BEV intensity image using vehicle dynamics, corresponding to 0.5 seconds of \lidar{} scan. In such a short time drift is negligible. }
\slwang{Our ground-truth poses are acquired
through an expensive yet accurate offline matching procedure. This provides accurate ground-truth with up to several centi-meter uncertainty.}

The aggregated \lidar{} points are rasterized into the \lidar{} intensity
image. Both the online intensity image and the intensity map are discretized at
a spatial resolution of 5cm covering a $30m\times24m$ region. During matching, we use the same spatial
resolution, plus a rotational resolution of 0.5\degree, with a total search 
range of 1m $\times1m\times2.5$\degree\   around the dead reckoning pose.


We report the median error of the localization over
all testing sequences compared to the ground truth, as well as the
failure rate. We define localization error over 50cm \slwang{at or before a certain traveling distance} as
``failure''. The median error \slwang{ at the end of each sequence} reflects how accurate the localization is
in the majority of cases while the failure rates reflect the worst case
performance. \slwang{In addition to those per sequence metric, we also plot the per frame cumulative localization error curve in \fref{fig:qual-cum}}.


\renewcommand{\arraystretch}{1.2}


\begin{table}[t]
  \centering
  \caption{Localization Performance on \textbf{Highway-LidarA} Dataset (Per Sequence) \label{tab:main-quantitative}}
   \begin{tabular}{cc|ccc|ccc}
\hline
     & & \multicolumn{3}{|c|}{\textbf{Median Error (cm)}}
     & \multicolumn{3}{|c}{\textbf{Failure Rate (\%)}} \\
     \textbf{Method} & Has $E_\textsc{dyn} ? $ & Lateral & Longitudinal
                     & Total
                     & $\le 100$m & $\le 500$m &$\le$ End
     \\\hline
Dynamics Only & Yes & 439.21 & 863.68 & 1216.01 & 0.46 & 98.14 & 100.00  \\
Raw Intensity & Yes & 1245.13 & 590.43 & 1514.42 & 1.84 & 81.02 & 92.49  \\
ICP & Yes &  \textbf{1.52} & 5.04 & \textbf{5.44} & 3.50 & 5.03 & 7.14  \\ \hline
Ours (FCN) & No & 5.27 & 4.10 & 7.71 & 1.41 & 6.13 & 12.44  \\
Ours (FCN) & Yes & 4.98 & \textbf{3.75} & 6.87 & 0.99 & 3.47 & 4.02  \\
Ours (LinkNet) & No & 4.84 & 4.65 & 8.09 & 1.89 & 1.90 & 1.92  \\
Ours (LinkNet) & Yes &4.80 & 4.61 & 7.75 & \textbf{0.46} & \textbf{0.46} & \textbf{0.47}  \\
\hline
     \end{tabular}
\end{table}


\renewcommand{\arraystretch}{1.1}
\begin{figure*}[t]
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
\multicolumn{3}{c}{\includegraphics[width=0.98\linewidth, trim={0 0 0 0}]{figure/transfer.pdf}} \\   
\\\end{tabular}
  \caption{A comparison between the two \lidar{} sensors: left: the different intensity profiles of their sweeps over the same location; right: the colormapped intensity image.}
  \label{fig:sensor-transfer}
\end{figure*}

\begin{table}[t]
  \centering
  \caption{Localization Performance on \textbf{Misc-LidarB} trained on \textbf{Highway-LidarA} (Per Sequence) \label{tab:main-transfer}}
   \begin{tabular}{cc|ccc|ccc}
\hline
     & & \multicolumn{3}{|c|}{\textbf{Median Error (cm)}}
     & \multicolumn{3}{|c}{\textbf{Failure Rate (\%)}} \\
     \textbf{Method} & Has $E_\textsc{dyn} ? $ & Lateral & Longitudinal
                     & Total
                     & $\le 100$m & $\le 500$m &$\le$ End
     \\ \hline

  Dynamics Only & Yes & 195.73 & 322.31 & 468.53 & 6.13 & 68.66 & 84.26  \\
  ICP & Yes & \textbf{2.57} & 15.29 & 16.42 & 0.46 & 28.43 & 37.53  \\ \hline
  Ours (Transfer) & Yes & 6.95 & \textbf{6.38} & \textbf{11.73} & \textbf{0.00}
                  & \textbf{0.71} & \textbf{1.95}  \\
  \hline
     \end{tabular}
\end{table}




\paragraph{Competing Algorithms} We experiment with two configurations of embedding networks. The first one,
\slwang{denoted as FCN}, uses the shallow network described
in Section~\ref{sec:robust-localization} for both online and map branches. 
\slwang{We also experiment the same matching network with/without the dynamic prior energy}
The second architecture uses a LinkNet~\cite{linknet} architecture for both the online and the
map branches.  We implement our networks with PyTorch 0.4. All the networks are trained using Adam over
four NVIDIA 1080Ti GPUs with initial learning rate at 0.001.  

We compare our algorithm against several baselines. \slwang{The raw matching baseline consists of performing the
matching-based localization in the similar manner of our proposed method but only use the
aggregated raw intensity BEV image and the map images, instead of the learned
embeddings. The ICP baseline conducts point to plane ICP between the raw 3D \lidar{} points against the 3D pre-scanned localization prior, initialized in the similar manner as us using the previous estimated location plus a vehicle dynamics move.}  



\paragraph{Localization Performance}
\tref{tab:main-quantitative} shows the resulting performance of competing algorithms on
our \textit{Highway-LidarA} test split.  \slwang{As shown from the table, our LinkNet based approach achieving best performance among all the competing algorithms in terms of failure rate. ICP is competitive in terms of median error, especially along lateral direction, but the failure rate is significant higher. Both dynamics and raw intensity matching will result in large drifts. Moreover, we've observed that deeper architecture and dynamic energy prior are general helpful in terms of achieving better performance. }
\fref{fig:qual-comparison} shows the localization error as
a function of the travel distance aggregated across all sequences from the
\textit{Highway-LidarA} test set with solid line being median and shaded region being the $95\%$ area, together with the distribution of lateral and
longitudinal errors per frame.  \slwang{From this figure we can see our approach is quite consistent in terms of travelling distances, across all frames.}
\fref{fig:qual-cum} compares our approach to ICP in terms of cumulative errors with $95\%$-percentile error reported. \slwang{From this we can see our method significantly outperform ICP in terms of the worst cases. }

\paragraph{Domain Shift}

\slwang{In order to showcase our proposed approaches are generalized and insensitive to \lidar{} sensors. We conduct the second experiment, where we train our network
on \textit{Highway-LidarA}, which is purely highway, collected using Lidar A on the test set of \textit{Misc-LidarB} which is highway + city collected on a different \lidar{} type B in a different state/province.   In order to better highlight the difference, in \fref{fig:sensor-transfer} we show two \lidar{}s intensity value distribution and their raw intensity image, collected at the same location. 
Finally,~\tref{tab:main-transfer} showcases the transfer performance of. From the table we can see our proposed neural network is able to generalize both across \lidar{} models, as well as across
environment types.}


\paragraph{Runtime Analysis}
\slwang{We conduct runtime analysis over both embedding networks and matching. 
Our LinkNet based embedding networks take roughly 70ms for a forward pass over both online
and map images. We also compared the \cudnn{} implementation of FFT-conv and standard spatial convolution. FFT gives over 13 times boost in terms of speed, reducing the runtime from $133ms$ to $9ms$ for a four-channel embedding. 
This enables us to run our localization algorithm at 15 Hz, achieving our real-time operation goal. 
}


\paragraph{Embedding Dimensions}
\slwang{
We also investigate the impact that the number of embedding channels has on matching performance and the runtime of the system. 
\tref{tab:ablation-channels} shows the performance. As shown in this table, increasing the number of channels does not lead a significant improved performance,
while reducing the number of channels could reduce the runtime of matching by a large margin, which favors relative low-dimensionality in practice.  
}




\begin{table}[t]
  \centering
  \caption{Localization performance under varying numbers of embedding channels
  \label{tab:ablation-channels}}
   \begin{tabular}{lrrrrrrrr}
     \toprule
       \textbf{Method}
       & \textbf{\shortstack{Matching top-5cm}}
     & \phantom{x}
     & \multicolumn{3}{c}{\textbf{Inference Time (ms)}}
     \\
     \cmidrule{4-6} & & & Backbone & Matching (Slow)
                                 &  Matching (FFT) \\
     \midrule
      Raw matching 	 & 13.95\% & & n/A	 	 & 32.33ms 	 & 3.18ms  	 \\
      1 channel 	 & 71.97\% & & 72.92ms 	 & 32.29ms 	 & 2.97ms  	 \\
      2 channels 	 & 72.08\% & & 72.03ms 	 & 65.42ms 	 & 5.09ms  	 \\
      4 channels 	 & 71.67\% & & 72.49ms 	 & 133.04ms 	 & 8.98ms  	 \\
      8 channels 	 & 71.63\% & & 74.32ms 	 & 272.18ms 	 & 16.87ms  	 \\
      12 channels 	 & 72.50\% & & 76.56ms 	 & 404.31ms 	 & 25.14ms  	 \\
     \bottomrule
     \end{tabular}
\end{table}








==> old_method.tex <==

\begin{figure}
  \centering
  \includegraphics[width=0.98\textwidth]{figure/teaser-v2.pdf}
  \caption{The full end-to-end architecture of our proposed deep localization network.}\label{fig:teasr}
\end{figure}

\section{Robust Localization Using \lidar{} Data}
\label{sec:robust-localization}

\newcommand{\cudnn}{cuDNN}



In this section, we discuss our %
\lidar{}  intensity 
localization system.  %
We first formulate
localization as an energy minimization problem and discuss each
energy term. We then present our real-time inference algorithm
followed by a description of how to train our model. %




\subsection{\lidar{} Localization as a Deep Structured Model}

We perform high-precision localization against pre-built \lidar{} intensity
maps. The maps are constructed from multiple passes through the same area,
which allow us to perform additional post-processing steps, such as dynamic
object removal. The accumulation of multiple passes also produces maps which
are much denser than individual \lidar{} sweeps. The maps are encoded as
orthographic bird's eye view (BEV) images of the ground. We refer the reader
to~\fref{fig:map-example} for a sample fragment of the maps used by our
system.





Let $\bx$ be the pose of the
self-driving vehicle (SDV). We assume that our  sensors are 
calibrated and neglect the effects of suspension, unbalanced tires, and
vibration. This enables us to simplify the vehicle's 6-DoF pose to only 3-DoF, namely a 2D translation and a heading angle, i.e., $\bx =
\{x, y, \theta \}$, where $x, y \in \mathbb{R}$ and 
$\theta \in (-\pi, \pi])$. 
At each time step $t$, our \lidar{} localizer takes as input the previous
pose $\bx\up$, the vehicle dynamics $\dot{\bx}^{(t)}$, the online \lidar{}
image $\cI\ut$, and the pre-built \lidar{} intensity map $\cM$. In
order to generate $\cI\ut$, we aggregate the $k$ most recent
\lidar{} sweeps using the IMU and wheel odometry. This
produces denser online \lidar{} images than just using the most recent sweep,
helping  localization. Since $k$ is small, drift is not an issue. 

We then  formulate the localization problem as an energy minimization
problem. We encode the fact that  the online sweep should be consistent with the map at the vehicle's
  location, and
the ego-motion corresponding to the new localization should be consistent 
  with the observation from the vehicle dynamics. Thus 
\begin{align}
  E_\textsc{loc}(\bx, \cI\ut, \cM; \bw)  & =  \elidar(\bx, \cI\ut, \cM; \bw)  + E_\dyn(\bx, \bx\up, \dot{\bx}^{(t)}), %
\end{align}
where $\bw$ is a set of learnable parameters and $ \bx\up  = \argmin_\bx E_\textsc{loc}(\bx, \cI\up, \cM; \bw)$. We now describe each
energy term in more detail.






\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/embeddings/online-4chan-deep-both}
    \caption{Online \lidar{} Image.}
  \end{subfigure}~
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/embeddings/emb-online-4chan-deep-both}
  \caption{Online embedding.}
  \end{subfigure}~
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/embeddings/map-4chan-deep-both}
    \caption{Intensity map.}
  \end{subfigure}~
  \begin{subfigure}[t]{0.24\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/embeddings/emb-map-4chan-deep-both}
  \caption{Map embedding.}
  \end{subfigure}~
  \caption{One example of the input and map embeddings.}
  \label{fig:embedding-example}
\end{figure}


\paragraph{\lidar{} Matching Energy:} Given a candidate pose $\bx$, our
\lidar{} matching energy $\elidar$ encodes the agreement between the current
online \lidar{} observation and the map indexed at the hypothesized 
pose $\bx$. To compute the energy, we first project both the map $\cM$ and the
online \lidar{} intensity image $\cI$ into an embedding space
using two deep neural networks. We then 
warp the online embedding according to a particular pose hypothesis, and
compute the cross-correlation between the warped online embedding and the
map embedding. Formally, this can be written as
\begin{equation}
  \elidar = s \left(\pi\left(f(\cI; \bw_\online), \bx\right), g(\cM; \bw_\map) \right),
\end{equation}
where $f(\cI; \bw_\online)$ and $g(\cM; \bw_\map)$ are the deep embedding networks of
the online \lidar{} image and the map, respectively, and
$\bw_o$ and $\bw_m$ are the networks' parameters.
$\pi$ represents a 2D rigid warping function meant to transform the online
\lidar{}'s embedding into the map's coordinate frame according to the given
pose hypothesis $\bx$. Finally, $s$ represents a cross-correlation operation
which takes into account the sparsity patterns of the input into account.
In particular, 
\begin{equation}
  s(\ba, \bb) = \frac{\left\langle 
    \ba \odot \left[ \cI \neq 0 \right],  \bb \odot \left[ \cM \neq 0 \right]
  \right\rangle}
  { \left\| \cI \right\|_0 \left\| \cM \right\|_0 }, %
\end{equation}
where $\odot$ represents an element-wise product, $\left[ \cdot \right]$
represents the Iverson bracket, and $\left\| \cdot \right\|_0$ the $\ell_0$-norm.





Our embedding functions $f(\, \cdot \, ; \bw_\online)$ and 
$g(\, \cdot \,; \bw_\map)$ are customized fully convolutional  neural networks.
The first branch $f(\, \cdot\, ; \bw_\online)$ takes as input the bird's eye view
(BEV) rasterized image of the $k$ most recent \lidar{} sweeps (compensated by ego-motion) and produces a
dense multi-channel representation at the same resolution as the input.
The second branch $g(\, \cdot \,; \bw_\map)$ takes as input a section of the 
\lidar{} intensity map, and produces an embedding with the same number of
channels as the first one, and the spatial resolution of the map.


\paragraph{Vehicle Dynamics Energy:} 
Our dynamics energy term encodes the
fact that the inferred vehicle velocity should agree with the
vehicle dynamics. In particular, wheel odometry and IMU are used as input to an extended Kalman filter to generate an estimate of the velocity of the vehicle. 
We then define the dynamics energy to be
\begin{equation} \label{eq:dynamics-energy}
E_\dyn =  \rho \left(\bx \ominus (\bx\up \oplus \dot{\bx}\ut)\right),
\end{equation}
with $\rho$  a robust error function and 
$\oplus$, $\ominus$ the 2D pose composition operator and inverse pose
composition operator respectively, which,
following~\citet{kummerle2009measuring} are defined as
\[
\mathbf{a} \oplus \mathbf{b} = 
\left[\begin{array}{c}
x_a + x_b \cdot \cos\theta_a - y_b \cdot \sin\theta_a \\
y_a + x_b \cdot \sin\theta_a + y_b \cdot \cos\theta_a\\
\theta_a + \theta_b 
\end{array}\right], 
\mathbf{a} \ominus \mathbf{b} = 
\left[\begin{array}{c}
(x_a - x_b) \cdot \cos\theta_b + (x_b - y_b) \cdot \sin\theta_b \\
-(x_a - x_b) \cdot \sin\theta_b + (x_b - y_b) \cdot \cos\theta_b \\
\theta_a - \theta_b 
\end{array}\right].
\]
In practice we choose $\rho$ to be a truncated quadratic error function
\begin{equation}
  \rho(\bz) = 
  \left\{
    \begin{aligned}
        & \bz^T \Sigma^{-1} \bz && \text{\ \ if\ \ } \bz \in \mathcal{R} \\ 
        & +\infty               && \text{\ \ otherwise \ \ }
    \end{aligned} \right.,
\end{equation}
 where $\Sigma$ is
the covariance matrix  and $\mathcal{R}$ is our three-dimensional search range.



\paragraph{Network Architectures:}
The $f$ and $g$ functions  are computed via multi-layer fully
convolutional neural networks. We experiment with a 6-layer network based on
the patch matching architecture used by \citet{luo2016efficient} and with
LinkNet by \citet{linknet}.
We use instance normalization~\citep{instancenorm} after each
convolutional layer \slwang{instead of batch norm, due to its capability of reducing instance-specific mean and covariance shift. Our embedding output has the same resolution as the input image, with a multi-dimensional embedding per pixel. The dimension is chosen based on the trade-off between performance and runtime. } %
We refer the reader to \fref{fig:embedding-example}
 for an illustration of one such channel. %

\begin{algorithm}[t]
  \caption{Online localization using the learned embeddings%
  \label{alg:online-localization}}
  \begin{algorithmic}[1]
    \Procedure{Localize}{$\bx\up$, $\dot{\bx}\ut$, $\cI^{(t)}$, $\cM\ut$}
    \State Get online \lidar{} embedding $f(\cI\ut; \bw_\online)$ as a feed-foward pass;
    \State Get map embedding $g(\cM\ut; \bw_\map)$ as a feed-foward pass;
    \State $E_\dyn \gets \bx\up \oplus \dot{\bx}\ut$ with
      Equation~\eqref{eq:dynamics-energy};
    \ForAll{$\theta_i \in \text{RotationCandidates}$}
    \State $E_\textsc{LiDAR}(i, :, :) \gets g(\cM\ut; \bw_\map) \ast
      \textsc{Rotate}(f(\cI\ut; \bw_\online), \theta_i)$ \label{alg:rotation} %
      \EndFor
      \State $\bx\ut \gets \argmax{\left( E_\textsc{LiDAR} + E_{\dyn} \right)}$;
    \EndProcedure
  \end{algorithmic}
\end{algorithm}

\subsection{Online Localization}

We estimate the pose of the SDV at each time step $t$ by solving 
\begin{equation}
  \min_{\bx} \elidar(\bx, \cI\ut, \cM; \bw)  + E_\dyn(\bx, \bx\up, \dot{\bx}\up).
\end{equation}
This is a complex non-linear and non-convex optimization over the continuous variable $\bx$. These type of problems are typically solved with non-linear iterative
solvers, which are sensitive to initialization and easily fall into local
minima. Moreover, most existing solvers have non-deterministic run times,
which is problematic for safety-critical real-time applications like
self-driving cars.


Instead, in this work we compute $\bx$ through a search-based method
which is much more efficient, given the characteristics of the problem.
To this end, we discretize the 3D search space over
$\bx = \{ x, y, \theta \}$ as a grid, and compute the term $E_\textsc{loc}$ for
every cell of our search space.
We center the  search space at the so-called dead reckoning pose, which
represents the pose of the vehicle at time $t$  estimated  
using  IMU and wheel encoders.
\slwang{The search range is selected in order to find a compromise between the
computational cost and the capability of handling large drift. }



The dynamic energy term $E_\dyn$ is a fixed
Gaussian score map centered around the dead reckoning pose, so it does not
have to be recomputed at every time step.
The most computationally demanding component of our model is
the fact that we need to enumerate all possible locations in our search
range. However, we observe that computing the inner product scores between
two 2D deep embeddings across all translational positions in our $(x, y)$
search range is equivalent to convolving the map embedding with the online
embedding as a kernel. This makes the search over $x$ and $y$ much faster to
compute. As a result, the entire optimization of $E_\textsc{loc}$ can be
performed using $n_\theta$ convolutions and one $\argmax$, where $n_\theta$
is the number of discretization cells in the rotation ($\theta$) dimension.








Therefore, we only need to run the embedding networks once, rotate the
computed online \lidar{} embedding $n_\theta$ times, and convolve each
rotation with the map embedding to get the scores for all the pose
hypotheses. Our solution is therefore globally optimal over our discretized
search space  including both rotation and translation. In practice,
the rotation of our online \lidar{} embedding is implemented using a spatial
transformer module~\cite{jaderberg2015spatial}, and generating all rotations
takes 5ms in total.
We refer the reader to Alg.~\ref{alg:online-localization} for a summary of  our proposed localization system. 

A naive GPU-based convolutional matching implementation is still \andreibc{too 
slow for our real-time operation goal}.
This is due to the fact that our ``convolution kernel'' is very large in
practice (in our experiments the size of our online \lidar{} embedding is
$301\times 241\times 4$). In order to speed this up, we perform this operation
in the Fourier domain, as opposed to the spatial one, according to convolution
theorem: $f \ast g = \cF^{-1}(\cF(f) \odot \cF(g))$, where ``$\odot$'' denotes
an element-wise product.
Theoretically, this reduces the complexity from $O(N^2)$ to $O(N\log N)$,
which translates to massive improvements in terms of run time, as we will
show in Section~\ref{sec:result}.











\subsection{Learning}

The localization system is end-to-end differentiable, enabling us to learn
all parameters jointly using back-propagation. We find that a simple cross-entropy
loss is sufficient to train the system, without requiring any additional, potentially
expensive terms, such as a reconstruction loss.
We define the cross-entropy loss between the ground-truth position and the
inferred score map as 
$
   \cL = -\sum_i \bp_{i, \text{gt}} \log \bp_i,
$
where the  labels $\bp_{i, \text{gt}}$ are represented as
one-hot encodings of the ground truth position, i.e., a tensor with
the same shape as the score map $S$, with a 1 at the correct pose. \slwang{ The
  covariance matrix of our dynamic energy term is determined empirically from
the difference between vehicle dynamics estimation and the GT position observed
in the training dataset. }







